Computer-aided proofs for multiparty computation with active security

Secure multi-party computation (MPC) is a general cryptographic technique that allows distrusting parties to compute a function of their individual inputs, while only revealing the output of the function. It has found applications in areas such as auctioning, email filtering, and secure teleconference. Given its importance, it is crucial that the protocols are specified and implemented correctly. In the programming language community it has become good practice to use computer proof assistants to verify correctness proofs. In the field of cryptography, EasyCrypt is the state of the art proof assistant. It provides an embedded language for probabilistic programming, together with a specialized logic, embedded into an ambient general purpose higher-order logic. It allows us to conveniently express cryptographic properties. EasyCrypt has been used successfully on many applications, including public-key encryption, signatures, garbled circuits and differential privacy. Here we show for the first time that it can also be used to prove security of MPC against a malicious adversary. We formalize additive and replicated secret sharing schemes and apply them to Maurer's MPC protocol for secure addition and multiplication. Our method extends to general polynomial functions. We follow the insights from EasyCrypt that security proofs can be often be reduced to proofs about program equivalence, a topic that is well understood in the verification of programming languages. In particular, we show that in the passive case the non-interference-based definition is equivalent to a standard game-based security definition. For the active case we provide a new NI definition, which we call input independence.

==> style/easycrypt.tex <==
%=======================================================================
% A listing mode for Easycrypt based on Assia Mahboubi's SSR

\lstdefinelanguage{Easycrypt} {

% Anything betweeen $ becomes LaTeX math mode
mathescape=true,
% Comments may or not include Latex commands
texcl=false,


% Vernacular commands
morekeywords=[1]{
admit, algebra, alias, apply, as,
assert, assumption, auto, axiom, axiomatized, beta, by, byequiv, byphoare, bypr, call, case,
cfold, change, class, clear, clone, congr, conseq, const, cut, declare, delta, do, done, eager,
elif, elim, else, end, equiv, exact, exfalso, exists, expect, export, fel, fieldeq, first,
fission, forall, fun, fusion, generalize, glob, goal, have, hint, hoare, hypothesis, idtac,
if, import, in, inline, instance, intros, iota, islossless, kill, last, left, lemma, let,
local, logic, modpath, module, move, nolocals, nosmt, of, op, phoare, pose, Pr, pr_bounded,
pred, print, proc, progress, proof, prover, qed, rcondf, rcondt, realize, reflexivity,
require, res, return, rewrite, right, ringeq, rnd, rwnormal, search, section, seq, sim,
simplify, skip, smt, sp, split, splitwhile, strict, subst, swap, symmetry, then, theory,
timeout, Top, transitivity, trivial, try, type, unroll, var, while, why3, with, wp, zeta}

% EC
morekeywords=[2]{forall, exists, fun},
% 'of' is removed from this list as it occurs in comments.

% Sorts
morekeywords=[3]{bool},

% tactics 
morekeywords=[4]{admit, algebra, alias, apply, assumption, auto, byequiv, byphoare, bypr, call, case, case-pl, cfold, change, clear, closing goals, congr, conseq, cut, done, eager, elim, elim*, exact, exfalso, exists, exists*, fel, fission, fusion, generalization, have, hoare, idtac, if, inline, introduction, kill, left, move, phoare, split, pose, proc, progress, rcondf, rcondt, reflexivity, rewrite, right, rnd, seq, sim, simplify, skip, smt, sp, split, splitwhile, subst, swap, symmetry, transitivity, trivial, unroll, while, wp},

% Terminators
morekeywords=[5]{
         by, done, exact, reflexivity, romega, smt, assumption, admit},


% Control
morekeywords=[6]{do, last, first, try, idtac, repeat},

% Various symbols
% For the ssr manual we turn off the prettyprint of formulas
 literate=
%       {->}{{$\rightarrow\ $}}2
%       {->}{{\tt ->}}3
	{<-}{{$\leftarrow\,$}}2
%       {<-}{{\tt <-}}2
%       {>->}{{$\mapsto$}}3
%       {<}{{$<\;\;$}}1
%       {<=}{{$\leq\;\;$}}1
%       {>=}{{$\geq\;\;$}}1
%       {<>}{{$\neq$}}1
%        {/\\}{{$\wedge\;\;$}}2
%        {\\/}{{$\vee\;\;$}}2
%       {^~}{{\textvisiblespace$\;\;$}}2
%       {~~}{{$\lnot\;\;$}}2
%       {<->}{{$\leftrightarrow\;$}}3
%       {<=>}{{$\Leftrightarrow\;$}}3
%       {:nat}{{$~\in\mathbb{N}$}}3
%	{fforall\ }{{$\forall_f\,$}}1
	{forall\ }{{$\forall\ \!$}}1
	{exists\ }{{$\exists\ \!$}}1
%       {MAPLE}{{\raisebox{-0.8cm}[0cm][0cm]{\hspace{18mm}\includegraphics[width=1cm]{maple}}}}1
	{^2}{{$^2$}}1
	{^3}{{$^3$}}1
	{^4}{{$^4$}}1
	{^5}{{$^5$}}1
	{^6}{{$^6$}}1
%       {negb}{{$\neg$}}1
%       {spp}{{:*:\,}}1
%       {~}{{$\sim$}}1
%       {\\in}{{$\in\;$}}1
%       {/\\}{$\land\,$}1
%       {:*:}{{$*$}}2
%	{=>}{{$\,\Rightarrow\ $}}1
%       {=>}{{\tt =>}}2
%       {:=}{{{\tt:=}\,\,}}2
%       {==}{{$\equiv$}\,}2
%       {!=}{{$\neq$}\ }2
%       {_cf0}{{$_{{0}}$}}1
%       {_cf1}{{$_{{1}}$}}1
%       {_cf2}{{$_{{2}}$}}1
%       {_cf0_0}{{$_{{00}}$}}1
%       {^-1}{{$^{-1}$}}1
%       {elt'}{elt'}1
%       {=}{{\tt=}\,\,}2
%       {+}{{\tt+}\,\,}2
,

% Comments delimiters, we do turn this off for the manual
%comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% String delimiters
morestring=[b]",

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=true,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,

% Default style fors listings
basicstyle=\ttfamily\footnotesize,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,

% do not eat spaces after) in inline
keepspaces=true,

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{dkviolet}},

% Style for gallina keywords
keywordstyle=[2]{\ttfamily\color{dkgreen}},

% Style for sorts keywords
keywordstyle=[3]{\ttfamily\color{lightblue}},

% Style for tactics keywords
keywordstyle=[4]{\ttfamily\color{dkblue}},

% Style for terminators keywords
keywordstyle=[5]{\ttfamily\color{red}},


%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
%commentstyle=\rmfamily,

}

